Probabilistic Bisimulation: Naturally on Distributions

In contrast to the usual understanding of probabilistic systems as stochastic processes, recently these systems have also been regarded as transformers of probabilities. In this paper, we give a natural definition of strong bisimulation for probabilistic systems corresponding to this view that treats probability distributions as first-class citizens. Our definition applies in the same way to discrete systems as well as to systems with uncountable state and action spaces. Several examples demonstrate that our definition refines the understanding of behavioural equivalences of probabilistic systems. In particular, it solves a long-standing open problem concerning the representation of memoryless continuous time by memory-full continuous time. Finally, we give algorithms for computing this bisimulation not only for finite but also for classes of uncountably infinite systems.

==> bisim.tex <==
\section{Probabilistic bisimulation on distributions}
\label{sec:bisim}

For the sake of readability we start with discrete systems, then we extend the setting to continuous systems.
%
For a set $S$, let $\dist(S)$ denote the set of simple distributions, i.e.\ functions $f:S\to[0,1]$ such that $f$ is non-zero for only finitely many elements $s_1,\ldots,s_n$ and $\sum_{i=1}^n f(x_i)=1$.
%
The set of \emph{probability measures} over $S$ (equipped with a $\sigma$-algebra clear from context) is denoted by $\measures(S)$.

\subsection{Discrete systems} 

Let us first define an important example of a formalism of discrete non-deterministic probabilistic labelled systems.

\begin{definition}
 \emph{Probabilistic automaton (PA, \cite{Segala:1996:MVR:239648})} is a triple $(\states, \labels, \patrans)$ where $\states$ is a finite set of \emph{states}, $\labels$ is a finite set of \emph{labels}, and $\patrans \; \subseteq \states \times \labels \times \dist(\states)$ is a finite \emph{probabilistic transition relation}.
\end{definition}

%A PA works similarly to a non-deterministic automaton. 
When in a state $\sta\in\states$, PA reads a label $\lab \in \labels$ and \emph{non-deterministically} chooses a successor distribution $\dis$ that is in the set of convex combinations over the set $\{\distwo \mid (s,\lab,\distwo) \in \patrans \}$, denoted by $s \patransa{\lab} \dis$. If there is no such distribution, the automaton halts. Otherwise, it moves into a successor state according to $\dis$. 
%
Considering convex combinations is necessary as it gives more power than pure resolution of non-determinism \cite{Segala:1996:MVR:239648}.
% 

A probabilistic automaton may also be viewed as a \emph{non-deterministic} labelled transition system over the uncountable space of probability distributions.
%
As each state supported by a probability distribution may have transitions for different labels, we need to work with arbitrary \emph{subsets} $\Lab\subseteq\labels$ of labels\jena{this is a bit fake argument}: we write $\sta \patransa{\Lab} \dis$ if $\sta \patransa{\lab} \dis$ for some $\lab\in\Lab$, and denote by $\states_\Lab := \{\sta \mid \exists \dis: \sta \patransa{\Lab} \dis\}$ the set of states having some label from $\Lab$.
%
For probability distributions $\dis, \distwo \in \dist(\states)$ and $\Lab \subseteq \labels$, we set $\dis \patransa{\Lab} \distwo$ if 
$\distwo = \frac{1}{\dis(\states_\Lab)}\sum_{\sta \in\states_\Lab} \dis(\sta) \cdot \distwo_\sta$
for some distribution $s \patransa{\Lab} \distwo_\sta$ for each $\sta \in \states_\Lab$.
%
Intuitively, we restrict in the transition to states that do not halt and consider all possible combinations of their transitions; we scale up by $\frac{1}{\dis(\states_\Lab)}$ to obtain a distribution again.


The natural bisimulation from this distribution perspective is as follows.

\begin{definition}\label{def:finite-bisim}
 Let $(\states, \labels, \patrans)$ be a PA and $R \subseteq \dist(\states) \times \dist(\states)$ be a symmetric relation. We say that $R$ is a (strong) \emph{probabilistic bisimulation} if for each $\dis \, R \, \distwo$ and $\Lab\subseteq\labels$
 \begin{enumerate}
  \item $\dis(\states_\Lab) = \distwo(\states_\Lab)$, and
  \item for each $\dis \patransa{\Lab} \dis'$ there is a $\distwo \patransa{\Lab} \distwo'$ such that $\dis' \, R \, \distwo'$.
 \end{enumerate}
%Furthermore, w
We set $\dis \bisim \distwo$ if there is a probabilistic bisimulation $R$ such that $\dis \, R \, \distwo$.
\end{definition}

\jena{Here, we were asked to formulate, whether it coincides with the standard non-deterministic bisimulation over the continuous transition system over probability distributions. This is hard to express because it is not clear how to formalize the non-deterministic system over distributions. Does it correspond to your co-algebra? Then yes.}





% \begin{example}
% In the system below, $s\bisim t$ as $s'\bisim \frac12t_1+\frac12t_1$.
% 
% \begin{tikzpicture}[outer sep=0.1em,->,xscale=1.1,
% state/.style={draw,circle,minimum size=1.7em,inner sep=0.1em}]
% \begin{scope}
% \node[state] (s) at (0,0.5) {$s$};
% \node[state] (s') at (1,0.5) {$s'$};
% \node[state] (u) at (2,1) {};
% \node[state] (v) at (2,0) {};
% \path[->] 
% (s) edge node[above] {$a$} node[below]{$1$} (s')
% (s') edge node[above]{\textonehalf} node[below]{$a$}(u)
% (s') edge node[below]{\textonehalf} (v)
% (u) edge[loop right] node[above]{$b$} node[right] {$1$} (u)
% (v) edge[loop right] node[above]{$c$} node[right] {$1$} (v)
% ;
% \end{scope}
% \begin{scope}[xshift=4cm]
% \node[state] (s) at (0,0.5) {$t$};
% \node[state] (s1) at (1,1) {$t_1$};
% \node[state] (s2) at (1,0) {$t_2$};
% \node[state] (u) at (2,1) {};
% \node[state] (v) at (2,0) {};
% \path[->] 
% (s) edge node[below] {$a$} node[above]{\textonehalf} (s1)
% (s) edge  node[below]{\textonehalf} (s2)
% (s1) edge node[above]{$a$} node[below]{$1$}(u)
% (s2) edge node[above]{$a$} node[below]{$1$}(v)
% (u) edge[loop right] node[above]{$b$} node[right] {$1$} (u)
% (v) edge[loop right] node[above]{$c$} node[right] {$1$} (v)
% ;
% \end{scope}
% \end{tikzpicture}
% 
% \end{example}

% 
% \begin{table}
% \begin{tabular}{ll}
%  probabilistic automata & $([0,1] \times \powerset(-))^A$ \\
%  Markov decision processes (MDP) & $([0,1] \times -)^A$ \\
%  unlabelled MDPs with deadlocks & $([0,1] \times \powerset(-))$ \\
%  Markov chain with deadlocks & $([0,1] \times -)$ \\
%  \hline
%  non-deterministic LTS & $(\powerset(-))^A$ \\
%  deterministic input-enabled LTS & $(-)^A$ \\
%  directed graphs & $\powerset(-)$ \\
%  deterministic runs & $(-)$ \\
% \end{tabular}
%  \caption{[S touto tabulkou moc nevim, co si pocit.]}
% \label{tab:bisim-subclasses}
% \end{table}


%Observe that the probabilistic bisimulation differs from the bisimulation on LTS only in requiring the same probability of reading each label; the functors differ exactly in providing this probability. \todo{tabulku jsem zatim zakomentoval, stejne nemame misto :)}

% Table~\ref{tab:bisim-subclasses} summarizes all relevant subclasses of PA and their corresponding functors and coinciding standard notions of bisimulation.


\subsection{Continuous systems} 

Let us now restate the definitions in the continuous setting.
By saying that a set $X$ is a \emph{measurable space}, we assume that it is equipped with a $\sigma$-algebra denoted by $\sigmafield(X)$.\footnote{We assume that the set of probability measures $\measures(X)$ over a measurable space $X$ is equipped with the Giry $\sigma$-algebra~\cite{giry1982categorical} $\statemeasuresfield$.} 
%In this subsection, $\powerset(-)$ denotes the functor returning for each measurable space $X$ the set $\powerset(X) = \sigmafield(X)$ of its measurable subsets. 
The following definition is similar to the treatment of~\cite{phd-cont}.

\begin{definition}
 A \emph{non-deterministic labelled Markov process} (NLMP) is a tuple $\pts = (\states, \labels, \{\kernel_\lab \mid \lab\in\labels\})$ where $\states$ is a measurable space of \emph{states}, $\labels$ is a measurable space of \emph{labels}, and 
 % with all sigletons $\{a\}$ for $a\in\labels$ measurable, and 
 $\kernel_\lab : \states \to \statemeasuresfield$ assigns to each state $\sta$ a measurable set of probability measures $\kernel_\lab(\sta)$ available in $\sta$ under $\lab$.%
%  
 \footnote{We further require that for each $\sta \in \states$ we have $\{(\lab,\mea) | \mea \in \kernel_\lab(\sta)\} \in \labelsfield \otimes \statemeasuresfield$ and for each $\Lab \in \labelsfield$ and $Y \in \statemeasuresfield$ we have $\{\sta\in\states \mid \exists \lab \in \Lab. \kernel_\lab(\sta) \cap Y \neq \emptyset \}\in \statesfield$.}
\end{definition}

The semantics is the same as before: when in a state $\sta$ a label $\lab$ is read, the system non-deterministically chooses a measure $\mea$ such that $\sta \patransa{\lab} \mea$, i.e. $\mea$ is in the set of convex combinations\footnote{The set of convex combinations is lifted to a measurable set $Z$ of measures over $\states$ as the set $\{\Sta \mapsto \int_{\mea\in Z} \mea(\Sta) \meatwo(d\,\mea)  \mid \text{$\meatwo$ is a measure over $Z$}\}$.} over $\kernel_\lab(\sta)$, or halts if there is no such measure.
% 
% Let us illustrate the definition by a system with $\states = \labels = [0,1]$ where for each state $\sta$ we have $\kernel_\sta(\sta) = \{\mea_{\leq \sta}, \mea_{\geq \sta}\}$ where $\mea_{\leq \sta}$ is the uniform distribution on $[0,\sta]$ and $\mea_{\geq \sta}$ is the uniform distribution on $[\sta,1]$. This system in a state, say $0.14$, can only read the label corresponding to the state, i.e. $0.14$ and then it chooses non-deterministically whether to move to a random lower state or a random greater state.
\begin{example}\label{ex:cont}
Consider a random number generator that also remembers its last number. We set $\labels=[0,1]$, $\states = [0,1]\times[0,1]$ and $\kernel_{x}(\langle \textit{new},\textit{last}\rangle) = \{\mea_{x}\}$ for $x=\mathit{new}$ and $\emptyset$ otherwise, where $\mea_{x}$ is the uniform distribution on $[0,1]\times \{x\}$. If we start with a uniform distribution over $S$ the measure of successors under any $x\in\labels$ is $0$. Thus in order to get any information of the system we have to consider successors under sets of labels, e.g.\ intervals.
\jena{This example motivates for something I tried to sneak in in the discrete world already. Needs to be changed.}
\end{example}

The distribution semantics is similar to the discrete setting. Reusing the notation, we set $\mea \patransa{\Lab} \meatwo$ if there is a measurable function $\resolver$ that to each state $\sta\in\states_\Lab$ assigns a measure $\meatwo_\sta$ such that $\sta \patransa{\Lab} \meatwo_\sta$.

\begin{definition}\label{def:infinite-bisim}
Let $(\states, \labels, \{\kernel_\lab \mid \lab \in \labels\})$ be a NLMP and $R \subseteq \measures(\states) \times \measures(\states)$ be a symmetric relation. We say that $R$ is a (strong) \emph{probabilistic bisimulation} if for each $\mea \, R \, \meatwo$ and measurable $\Lab\subseteq\labels$
 \begin{enumerate}
  \item $\mea(\states_\Lab) = \meatwo(\states_\Lab)$, and
  \item for each $\mea \patransa{\Lab} \mea'$ there is a $\distwo \patransa{\Lab} \meatwo'$ such that $\mea' \, R \, \meatwo'$.
 \end{enumerate}
We set $\dis \bisim \distwo$ if there is a probabilistic bisimulation $R$ such that $\dis \, R \, \distwo$.
\end{definition}

%The use of the same symbol $\bisim$ for both bisimulation in the finite and the general case is justified by the following observation.

%\addtocounter{aux}{1}

%\begin{proposition}\label{prop:coin-on-pa}
%The bisimulations of Definition~\ref{def:finite-bisim} and Definition~\ref{def:infinite-bisim} coincide on PA.
%\end{proposition}
% \begin{proof}[Proof idea]
% For a PA understood as $\functorinf$-coalgebra with discrete $\Sigma(\labels)$, the behaviour under $A\in\Sigma(\labels)$ is just a ``sum'' of behaviours under $\{a\}$ for each $a\in\labels$.
% \end{proof}

%Let us note that $\functorinf$ is the appropriate functor for the distribution bisimulation. The functor $\functorfin$ is only an (important) specialization.

\begin{example}\label{ex:cont2}
 Considering Example~\ref{ex:cont}, states $\{x\}\times[0,1]$ form a class of $\bisim$ for each $x\in[0,1]$ as the old value does not affect the behaviour. More precisely, $\dis\bisim\distwo$ iff marginals of their first component are the same.
 \jena{this needs to get updated}
\end{example}


\subsection*{Coalgebraic definitions}

Our definition of bisimulation is not created ad-hoc, but is actually an instantiation of the standard bisimulation for a particular \emph{coalgebra}. Although this aspect is not necessary for understanding the paper, it is another argument for naturalness of our definition. For reader's convenience, we present a short introduction to coalgebras and the formal definitions in Appendix. Here we only provide an intuitive explanation by example.

Usual non-deterministic labelled transition systems are essentially given by the transition function $\states\to \powerset(\states)^\act$. Indeed, given a state $s\in \states$ and a label $a\in\act$, we can obtain the set of the successors $\{s'\in\states\mid s\tran{a}s'\}$. This coalgebra induces a bisimulation which coincides with the classical one of Park and Milner \cite{DBLP:books/daglib/0067019}. Similarly, probabilistic automata are given by the transition function $\states\to \powerset(\dist(\states))^\act$ as instead of successors there are distributions over successors. And again the corresponding coalgebraic bisimulation can be shown to coincide with the classical ones of Larsen and Skou~\cite{DBLP:conf/popl/LarsenS89} and Segala \cite{}.

In contrast, our definition can be obtained by considering states $\states'$ to be distributions $\dist(S)$ over the original state space and defining the transition function to be $\states'\to ([0,1]\times\powerset(\states'))^\act$. The difference to the standard non-probabilistic case is that for each label we also know the mass of the current state distribution that can perform this label. 
\todo{Jan: comment on the standard non-deterministic bisimulation over the continuous transition system over probability distributions?} 
In the continuous case, the trasnition function is $\states'\to ([0,1]\times\powerset(\states'))^{\Sigma(\act)}$ as we need to consider all measurable sets of labels, i.e.\ all elements of $\Sigma(\act)$.






==> discuss.tex <==
\section{Discussion}
\label{sec:discuss}

\subsection{Bisimulation coalgebraically}

Definitions of bisimulations can be given in terms of relations and we will do so, too. However, for two reasons we will also give a coalgebraic definition that induces our relational definition. Firstly, due to the general framework our definition will cover a spectrum of bisimulations depending on the interpretation of the coalgebra and is applicable to more complex systems, automatically yielding the bisimulation definitions. Secondly, any ad-hoc features of a simple coalgebraic definition are more visible and can be clearly identified, whereas it is difficult to distinguish which of two similar relational definitions is more natural. As we assume no previous knowledge of categorical notions we give a brief introduction to coalgebras in the spirit of \cite{Sangiorgi:2011:ATB:2103601}.


A \emph{functor} $F$ (on sets) assigns to each set $X$ a set $F(X)$, and to each set function $f:X\to Y$ a set function $F(f):F(X)\to F(Y)$ such that two natural conditions are satisfied: (i) the identity function on $X$ is mapped to the identity function on $F(X)$ and (ii) a composition $f\circ g$ is mapped to a composition $F(f)\circ F(g)$.

\begin{example}
The powerset functor $\powerset(-)$ maps a set $X$ to the set $\powerset(X)$ of its subsets and a function $f:X\to Y$ to $\powerset(f):\powerset(X)\to\powerset(Y)$ by $U\mapsto \{f(x)\mid x\in U\}$. 

Similarly, for a fixed set $\act$, the operator $(-)^\act$ mapping $X$ to the set $X^\act$ of functions $\act\to X$ is a functor, where the image of $f:X\to Y$ is $F(f):X^\act\to Y^\act$ given by mapping $u:\act\to X$ to $f\circ u:\act\to Y$.
\end{example}

For a functor $F$, an \emph{$F$-coalgebra} is a pair of the carrier set (or state space) $S$ and the operation function $\nxt:S\to F(S)$. Intuitively, the function $\nxt$ describes the transition to the next step.

\begin{example}
A transition system $(S,\rightarrow)$ with $\mathord{\rightarrow}\subseteq S\times S$ can be understood as a $\mathcal P(-)$-coalgebra by setting $\nxt(s)=\{s'\mid s\tran{} s'\}$. And vice versa, every $\mathcal P$-coalgebra gives rise to a transition system.

A labelled transition system $(S,\act,\rightarrow)$ with the set of labels $\act$ and $\mathord{\rightarrow}\subseteq S\times \act\times S$ can be seen as a $(\powerset(-))^\act$-coalgebra with $\nxt:S\to (\powerset(S))^\act$ given by $\nxt(s)(a)\to \{s'\mid s\tran{a}s'\}$.
\end{example}


A \emph{bisimulation} on an $F$-coalgebra $(S,\nxt)$ is a an $F$-coalgebra $(R,\overline\nxt)$ with $R\subseteq S\times S$ such that the two projections $\pi_1:R\to S$ and $\pi_2:R\to S$ make the following diagram commute:\footnote{I.e.\ $\nxt\circ\pi_1=F(\pi_1)\circ\overline\nxt$ and $\nxt\circ\pi_2=F(\pi_2)\circ\overline\nxt$.}

\begin{tikzpicture}[x=2.5cm,y=1.2cm]
\node (S1) at (-1,0) {$S$};
\node (FS1) at (-1,-1) {$F(S)$};
\node (S2) at (1,0) {$S$};
\node (FS2) at (1,-1) {$F(S)$};
\node (R) at (0,0) {$R$};
\node (FR) at (0,-1) {$F(R)$};
\path[->] (S1) edge node[left] {$\nxt$} (FS1)
	  (S2) edge node[right] {$\nxt$} (FS2)
	  (R) edge node[left] {${\overline\nxt}$} (FR);
\path[->] (R) edge node[above] {$\pi_1$} (S1)
	  (R) edge node[above] {$\pi_2$} (S2)
	  (FR) edge node[below] {$F(\pi_1)$} (FS1)
	  (FR) edge node[below] {$F(\pi_2)$} (FS2);
\end{tikzpicture}

\begin{example}
For LTS, the coalgebraic bisimulation coincides with the classical one of Park and Milner \cite{DBLP:books/daglib/0067019}, where a symmetric $R$ is a bisimulation if for every $sRt$ and $s\tran{a}s'$ there is $t\tran{a}t'_{s,a,s',t}$ with $s'Rt'_{s,a,s',t'}$. Indeed, given a classical bisimulation $R$, one can define $\nxt(\langle s, t\rangle)$ for $a\in \act$ to contain for every $s\tran{a}s'$ the matching pair $\langle s',t'_{s,a,s',t}\rangle$ and symmetrically for $t$. Since all these pairs are from $R$, $(R,\overline\nxt)$ is indeed a coalgebra. Further, the projection $F(\pi_1)$ of $\nxt(\langle s, t\rangle)$ yields all and nothing but the successors of $s$, symmetrically for $t$, hence the commuting. 

Conversely, given a coalgebraic bisimulation $(R,\overline\nxt)$, the commuting of $\pi_1$ guarantees that $\nxt(\langle s, t\rangle)$ yields all and nothing but the successors of $s$. Hence, for each $s\tran{a}s'$ there must be $\langle s',t'\rangle\in\nxt(\langle s, t\rangle)\subseteq R$, moreover, with $t\tran{a}t'$ due to $\pi_2$ commuting.
\end{example}

\medskip

As we have seen, the coalgebraic definition coincides with the relational one for non-probabilistic systems. One can use the same theory for finite probabilistic systems, too. Let $\dist(X)$ denote the set of simple distributions, i.e.\ functions $f:X\to[0,1]$ such that $f$ is non-zero for only finitely many elements $x_1,\ldots,x_n$ and $\sum_{i=1}^n f(x_i)=1$. Note that $\dist(-)$ can be understood as a functor. 

\begin{example}
We can interpret $(\dist(-)\cup\{\cannot\})^\act$-coalgebras as finite Markov decision processes $(S,\act,Pr)$ with $Pr:S\times \act\to\dist(S)\cup\{\cannot\}$ that under each action either proceed to a distribution on successors (as opposed to a non-deterministic choice in LTS) or not have the action available (the special element $\cannot$). The corresponding coalgebraic bisimulation can be shown to coincide with the classical one of Larsen and Skou~\cite{DBLP:conf/popl/LarsenS89}, where an equivalence relation $R$ is a bisimulation if $\sum_{u\in U}Pr(t,a)(u)=\sum_{u\in U}Pr(t',a)(u)$ for every $a\in \act$, classes $T,U$ of $R$ and $t,t'\in T$.
\end{example}

In contrast, uncountable probabilistic systems are more intricate. The set of \emph{probability measures} over $X$ (equipped with a $\sigma$-algebra clear from context) is denoted by $\measures(X)$.
Again, defining $\measures(f)(\mu)=\mu\circ f^{-1}$ makes $\measures(-)$ into a functor.

\begin{example}
We can interpret $\measures(-)$-coalgebras as Markov chains with general (possibly uncountable) state space. However, it is intricate to prove that the corresponding bisimulation is defined so that it coincides with the relational definition as already mentioned in Section~\ref{sec:intro}. 
%One can restrict to ultramteric state spaces, which do not include even $\Rset$~\cite{DBLP:conf/icalp/VinkR97}. In order to obtain general results, one has to use a construction~\cite{DBLP:journals/mscs/Edalat99}, which is ``ingenious and intricate and invloved moving between two closely related categories''~\cite{Sangiorgi:2011:ATB:2103601} or use ``powerful techniques like measurable selection theorems''~\cite{DBLP:conf/icalp/Doberkat03}.\todo{vic odkazu ze slozite}
\end{example}

In the following section, the proposed bisimulation is induced by a different view on the probabilistic systems. Namely, we consider distributions $\dist(S)$ or measures $\measures(S)$ over its state space $\states$ to form the carrier of the coalgebra. A transition then changes this distribution. For instance, a Markov chain can be seen this way as a coalgebra of the identity functor.


\subsection{Bisimulation on distributions coalgebraically}

Observe that from the state-based point of view PA correspond to $(\powerset(\dist(-)))^\labels$-coalgebras.%\todo{functor $\powerset$ by mel vracet jen konecny podmnoziny, ve spojitym pripade to budou zase jen meritelny podmnoziny}

---

In order to capture the distributional semantics of PA and other systems, we define a functor for finite probabilistic systems with non-determinism by\footnote{On function, we define the functor by $\functorfin(f)(n)(a)=(id\times\powerset(f))(n(a))$.}
\begin{align*}
\boxed{ ([0,1] \times \powerset(-))^\labels  \tag{$\functorfin$}}
\end{align*}

Now a PA $(\states, \labels, \patrans)$ is a $\functorfin$-coalgebra %of the functor
with the carrier set $\dist(\states)$. Indeed, the coalgebra assigns to a distribution $\dis$ and a label $\lab$ the pair $(p,\Dis)$ where 
\begin{itemize}
 \item $p= \dis(\states_\lab)$ is the probability of states that can read $\lab$;
%  \item $\Dis = \convex(\{\dis' \mid \dis \patransa{\lab} \dis' \})$ is the set of convex combinations of successor distributions where we set $\dis \patransa{\lab} \dis'$ if $\dis(\states_\lab) > 0$ and if for each $\sta\in\states_\lab$ we have $\sta \patransa{\lab} \distwo_\sta$ such that $\dis' = \sum_{\sta \in\states_\lab} \frac{\dis(\sta)}{\dis(\states_\lab)} \cdot \distwo_\sta$.%, and $\convex$ takes a convex combination of a set of distributions.
% 
% Honzovo?
% \item $\Dis = \convex\{\sum_{\sta \in\states_\lab} \frac{\dis(\sta)}{\dis(\states_\lab)} \cdot \distwo_\sta \mid \forall \sta\in\states_\lab:\sta \patransa{\lab} \distwo_\sta,$ $\dis(\states_\lab) > 0\}$ is the set of convex combinations of successor distributions. We write $\dis \patransa{\lab} \dis'$ for every $\dis'\in \Dis$.
% 
% moje take 2
\item $\Mea = \emptyset$ if $\mea(\states_\lab) = 0$, and $\Mea$ is the set of convex combinations over $\{\frac{1}{\dis(\states_\lab)}\sum_{\sta \in\states_\lab} \distwo_\sta \cdot \dis(\sta) \mid \forall \sta\in\states_\lab.\sta \patransa{\lab} \distwo_\sta\}$, otherwise.
%  $$ \mea_\resolver(\Sta) = \frac{1}{\mea(\states_\Lab)} \cdot \int_{\sta\in\states} \resolver(\sta)(\Sta)\ \mea(d\sta) \quad \forall \Sta\in\statesfield.$$
We write $\dis \patransa{\lab} \dis'$ for every $\dis'\in \Dis$.
% 
% moje
% \item $\Dis = \{\dis' \mid \dis \patransa{\lab} \dis'\}$ is the set of successor distributions where we define $\dis \patransa{\lab} \dis'$ if $\dis(\states_\lab) > 0$ and if $\dis' \in 
% \convex\{\frac{1}{\dis(\states_\lab)} \sum_{\sta \in\states_\lab} \dis(\sta) \cdot \distwo_\sta \mid \forall \sta\in\states_\lab:\sta \patransa{\lab} \distwo_\sta\}$. Here, $\convex(X)$ denotes the set of convex combinations over $X$. 
% 
In other words, $M$ is obtained by restricting $\mu$ to the states that can read $\lab$ and weighting all possible combinations of their transitions. % accordingly.
\end{itemize}



Although we can use $\functorfin$ to capture the distribution semantics of PA as above, we could as well use it differently:
%\footnote{Alternatively, 
if we defined that a label that cannot be read in the current state is  \emph{ignored} instead of halting, the successor distribution would be defined by making a step from states that can read the label and staying elsewhere. (This approach is discussed in the next section.) %\todo{ten footnote bych vyhodil} 
Moreover, we could easily extend the functor to systems with real rewards (as in~\cite{DBLP:conf/ijcai/CastroPP09}) %\todo{lze i Cost...HH+Andrea} 
simply by adding $\Rset$ to get $\Rset\times([0,1] \times  \powerset(-))^\labels $ for rewards on states or $([0,1] \times \powerset(\Rset\times -))^\labels $ on transitions etc. Similarly, for systems without the inner non-determinism like Rabin automata, we could simplify the functor to $([0,1] \times -)^\labels$. The only important and novel part of the functor is $[0,1]$ stating the overall probability mass that performs the step. (This is also the only difference to non-probabilistic coalgebraic functors.)
% apart form the carrier now having structure $\measures(S)$.)
In all the cases, the generic $\functorfin$-bisimulation keeps the same shape. What changes is the induced relational bisimulation. 
% For PA as $\functorfin$-coalgebras this gives rise to the following:

----


\begin{lemma}\label{lem:fin-coin}
 The union of $\functorfin$-bisimulations %from Definition~\ref{def:finite-functor} 
and %the relational bisimulation 
$\bisim$ %s by Definition~\ref{def:finite-bisim} 
coincide.
\end{lemma}

----

Therefore, in order to capture the distributional semantics of NLMP and other continuous systems, we define a functor
\begin{align*}
 \boxed{([0,1] \times \powerset(-))^{\powerset(\labels)} } \tag{$\functorinf$}
\end{align*}
And again we could vary the functor and adapt it to our particular needs. However, the vital part is now not only $[0,1]$, but also the use of measurable sets of labels instead of individual labels.

Analogously to the discrete case, %Definition~\ref{def:finite-functor}, 
we can view NLMP as $\functorinf$-coalgebras
%
%\begin{definition}\label{def:infinite-functor}
% A NLMP $\pts = (\states, \labels, \{\kernel_\lab \mid \lab\in\labels\})$ is a coalgebra of the functor
% 
with a carrier set $\measures(\states)$. The coalgebra assigns to $\mea \in \measures(\states)$ and to a set of labels $\Lab \in \labelsfield$ the pair $(p,\Mea)$ such that 
\begin{itemize}
 \item $p= \mea(\states_\Lab)$ is the measure of states that can read some $\lab\in\Lab$ where $\states_\Lab = \{ \sta\in\states \mid \exists \lab \in \Lab. \kernel_\lab(\sta) \neq \emptyset \}$;
%  
% Honzovo
%  \item $\Mea = \convex\{\mea_\resolver \mid \mea(\states_\Lab) > 0, \text{measurable }\resolver:\states_\Lab\to\bigcup_{\lab\in\Lab}\kernel_\lab  \}$  where $\convex$ is the measurable convex combination, again for $\mea'\in M$ we write $\mea \patransa{\Lab}\mea'$, and 
%  $$ \mea_\resolver(\Sta) = \frac{1}{\mea(\states_\Lab)} \cdot \int_{\sta\in\states} \resolver(\sta)(\Sta)\ \mea(d\sta) \quad \forall \Sta\in\statesfield.$$
%
% moje take 2
\item $\Mea = \emptyset$ if $\mea(\states_\Lab) = 0$, and $\Mea$ is the set of convex combinations\footnote{The set of convex combinations is lifted to a measurable set $Z$ of measures over $\states$ as the set $\{\Sta \mapsto \int_{\mea\in Z} \mea(\Sta) \meatwo(d\,\mea)  \mid \text{$\meatwo$ is a measure over $Z$}\}$.} over $\{\mea_\resolver \mid \text{measurable }\resolver:\states_\Lab\to\bigcup_{\lab\in\Lab}\kernel_\lab  \}$, otherwise, where
 $$ \mea_\resolver(\Sta) = \frac{1}{\mea(\states_\Lab)} \cdot \int_{\sta\in\states} \resolver(\sta)(\Sta)\ \mea(d\sta) \quad \forall \Sta\in\statesfield.$$
%
% 
% moje:
%  \item $\Mea = \{\mea' \mid \mea \patransa{\Lab} \mea'\}$ where we set $\mea \patransa{\Lab} \mea'$ if $\mea(\states_\Lab) > 0$ and if there is a measurable function $\resolver$ that assigns to each $\sta \in \states_\Lab$ a probability measure over $\{(\lab,\mea) \mid \lab\in\Lab, \mea \in \kernel_\lab(\sta)\}$ such that $R(s) = \int_{(\lab,\mu) \in \Lab \times \measures(\states)} \mu \rho(s) (d\,(a,\mu))$ and
% %  
% %  $\mea' = \convex\{\mea_\resolver \mid \text{measurable }\resolver:\states_\Lab\to\bigcup_{\lab\in\Lab}\kernel_\lab  \}$  where $\convex$ is the measurable convex combination, again for $\mea'\in M$ we write $\mea \patransa{\Lab}\mea'$, and 
%  $$ \mea(\Sta) = \frac{1}{\mea(\states_\Lab)} \cdot \int_{\sta\in\states} \resolver(\sta)(\Sta)\ \mea(d\sta) \quad \forall \Sta\in\statesfield.$$
\end{itemize}
%\end{definition}

----


\begin{lemma}\label{lem:inf-coin}
The %greatest 
union of $\functorinf$-bisimulations and $\bisim$ coincide.
% The coalgebraic bisimulations from Definition~\ref{def:infinite-functor} and the relational bisimulations by Definition~\ref{def:infinite-bisim} coincide.
\end{lemma}


==> intro.tex <==
\section{Introduction} 
\label{sec:intro}

The theory of bisimulations is a well-established and elegant framework to describe equivalence between processes based on their behaviour. The original definition was given for non-deterministic processes \cite{DBLP:conf/tcs/Park81,DBLP:books/daglib/0067019} and was further extended to finite probabilistic systems in \cite{DBLP:conf/popl/LarsenS89}. Since then many variants of bisimulations have been proposed and investigated, in particular an extension to non-deterministic probabilistic systems \cite{DBLP:conf/concur/SegalaL94}. Recently, there has been considerable interest in regarding probabilistic systems as deterministic transformers of probability \emph{distributions} rather than individual stochastic processes \cite{DBLP:conf/qest/KorthikantiVAK10,DBLP:conf/lics/AgrawalAGT12,DBLP:journals/corr/0001MS13a}. In the standard semantics, of probabilistic systems, when a probabilistic step from a state to a distribution is taken, the random choice is resolved and we continue from one of the successor states. In contrast, under the \emph{distribution semantics} the choice is not resolved and we continue from the distribution over successors. Thus, instead of the current state the transition changes the current distribution over the states. Although the distribution semantics is very natural in many contexts \cite{DBLP:dblp_journals/fac/Hennessy12}, it has been only partially reflected in the study of bisimulations \cite{DBLP:dblp_journals/fac/Hennessy12,DBLP:journals/ijfcs/DoyenHR08,DBLP:journals/corr/FengZ13}.

In this paper, we give a \emph{natural} definition of such bisimulations. 
It arises as an unusual, but very simple instantiation of the standard coalgebraic framework for bisimulations \cite{Sangiorgi:2011:ATB:2103601}. (No knowledge of coalgebra is required from the reader though.) Despite its simplicity, the resulting notion is surprisingly fruitful for two reasons. 

Firstly, it is more precise than other equivalences when applied to systems with the distribution semantics such as large-population models where different parts of the population act differently \cite{may1974biological}. Indeed, as argued in \cite{DBLP:journals/fac/GeorgievskaA12}, some equivalent states are not identified in the standard probabilistic bisimulations and too many are identified in the recent distribution based bisimulations \cite{DBLP:journals/ijfcs/DoyenHR08,DBLP:journals/corr/FengZ13}. Our approach allows for a bisimulation identifying precisely the desired states~\cite{DBLP:journals/fac/GeorgievskaA12}. 

Secondly, 
% although we define bisimulation on probabilistic systems under the distribution semantics, it yields not only an equivalence on distributions, but also induces an equivalence on states being Dirac distributions. 
% The latter equivalence is thus a novel bisimulation on the systems with the standard semantics. 
our bisimulation over distributions induces a novel behavioural equivalence on states.
This equivalence is useful, for it identifies states that are behaviourally indistinguishable in many settings, but were unnecessarily distinguished by standard bisimulations. We document this in several applications: ranging from partially observed systems control \cite{DBLP:journals/aamas/ShaniPK13} where the controller only has a probabilistic belief where the system is, over distributed scheduler synthesis  \cite{DBLP:conf/concur/GiroDF09}, to continuous-time systems where random waiting times are sampled, but are not observed before they elapse \cite{DBLP:journals/iandc/DArgenioK05}.
% Both views on the bisimulation yield a fruitful equivalence notion and 
%We devote Section~\ref{sec:applications} to explaining these applications and here only sketch 
We illustrate this in the following intriguing example from the continuous-time area due to \cite{holger-christel}.

\begin{example}\label{ex:intro}
Consider the following two stochastic automata (formally defined in Section \ref{sec:bisim}). They have ``kitchen timers'' $x$ and $y$, which get a random exponentially distributed value when a state with a corresponding assignment is entered. Then the time elapses and the values of the timers decrease until the first one reaches $0$. Then a transition to the next state is taken and the other timers keep on running.

\begin{center}
\myspace
\begin{tikzpicture}[outer sep=0.1em,->,
state/.style={draw,circle,minimum size=1.7em, inner sep=0.1em},
label/.style={font=\small}]


\begin{scope}
\node (s) at (0,2) [state] {$\loctop$};
\node (t) at (-1,1) [state] {$\locleft$};
\node (u) at (1,1) [state] {$\locright$};
\node (v) at (0,0) [state] {$\locbottom$};
\node (ss) at (1,2.1) {$\substack{x:=\ex(1),\\y:=\ex(2)}$};

\path[->]
(s) edge node[label,right]{$a$} node[label,left]{$x=0$} (t)
(s) edge node[label,left]{$b$} node[label,right]{$y=0$} (u)
(t) edge node[label,right]{$b$} node[label,left]{$y=0$} (v)
(u) edge node[label,left]{$a$} node[label,right]{$x=0$} (v)
;
\end{scope}

\begin{scope}[xshift=4.6cm]
\node (s) at (0,2) [state,inner sep=0em] {$\loctop'$};
\node (t) at (-1,1) [state,inner sep=0em] {$\locleft'$};
\node (u) at (1,1) [state,inner sep=0em] {$\locright'$};
\node (v) at (0,0) [state,inner sep=0em] {$\locbottom'$};
\node (ss) at (1,2.1) {$\substack{x:=\ex(1),\\y:=\ex(2)}$};
\node (tt) at (-2,1) {$\substack{\\y:=\ex(2)}$};
\node (uu) at (2,1) {$\substack{\\x:=\ex(1)}$};

\path[->]
(s) edge node[label,right]{$a$} node[label,left]{$x=0$} (t)
(s) edge node[label,left]{$b$} node[label,right]{$y=0$} (u)
(t) edge node[label,right]{$b$} node[label,left]{$y=0$} (v)
(u) edge node[label,left]{$a$} node[label,right]{$x=0$} (v)
;
\end{scope}
\end{tikzpicture}
\myspace
\end{center}

\noindent
If we observe the times when transitions occur (a timer rings), the two systems behave the same. Indeed, due to the memoryless property of the exponential distributions, there is no way to distinguish them. Yet existing notions of bisimulations and behavioural equivalences in the literature fail to capture this. The distributional view, which we take, is necessary here. Indeed, as $\locleft'$ cannot be matched by any $\locleft$ with a particular remaining time on the timer, but can be matched by an appropriate distribution over $\locleft$'s with all possible remaining times. See Section \ref{sec:applications} for details.
\end{example}

Nevertheless, the key idea to work with distributions instead of single states also bears disadvantages. The main difficulty is that even for finite systems the space of distributions is uncountable, thus bisimulation is difficult to compute. However, we show that it admits a concise representation using methods of linear algebra and we give algorithms to compute it.
Further, in order to cover e.g.\ continuous-time systems, we need to handle both uncountably many states (that store the sampled time) and labels (real time durations). Fortunately, there is an elegant way to do so using the standard coalgebra framework. Moreover, it can easily be further generalized, e.g.\ adding rewards to the generic definition is a trivial task.

\noindent \textbf{Our contribution} is the following:
\begin{itemize}
 \item We give a natural definition of bisimulation from the distributional perspective for systems with generally uncountable spaces of states and labels.
 \item We argue on several applications that the definition is more useful in many settings than the classical notions of probabilistic bisimulation.
% (including distributed or partial-observation control, large-population models, or continuous-time systems).
 \item We give the first algorithm to compute distributional bisimulation on finite non-deterministic probabilistic systems and, further, an algorithm deciding bisimilarity on several classes of uncountable (continuous-time) systems.
\end{itemize}

% \noindent \textbf{Outline} 
% Section \ref{sec:defs} introduces the notion of coalgebra together with a notion of the corresponding bisimulation. In Section \ref{sec:bisim} we define our bisimulation both using a simple coalgebraic description as well as in a standard relational way. Section \ref{sec:applications} gives further reasons %for naturalness and 
% to study this bisimulation by means of several application. In Section \ref{sec:algorithms} the algorithms to compute the bisimulation are given. For reader's convenience, in each section we first explain the ideas on the finite case and then move to the general case. Due to space constraints full proofs and other supplementary material can be found in \cite{myproofs}.






==> macros.tex <==

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\usepackage{amssymb,amsmath,amsfonts}
\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage{amsthm}
%\let\proof\IEEEproof
%\newtheorem{aux}{Aux}
%\newtheorem{theorem}{Theorem}%[section]
%\newtheorem{lemma}[aux]{Lemma}
%\newtheorem{corollary}[aux]{Corollary}
%\newtheorem{proposition}[aux]{Proposition}
%\newtheorem{fact}[aux]{Fact}
%\newtheorem{remark}[aux]{Remark}
%\newtheorem{conjecture}[aux]{Conjecture}
%\newtheorem{definition}[aux]{Definition}
%\newtheorem{claim}[aux]{Claim}

%\theoremstyle{definition}
%\newtheorem{example}[aux]{Example}


\newcommand{\citeapp}[1]{\cite{myproofs}}%{Appendix~\cite{#1}}

\usepackage{enumerate}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage{textcomp} %tilde
%\usepackage[all]{xy}

\usepackage{tikz,pgffor}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
\usetikzlibrary{automata}
\usetikzlibrary{decorations.pathmorphing} % for snake lines
\usetikzlibrary{decorations.pathreplacing} % for snake lines
\usetikzlibrary{calc} % for manimulation of coordinates

%%%%%%%%%%%%%%%%%%%% general math

\newcommand{\Nset}{\mathbb{N}}
\newcommand{\Nseto}{\Nset_0}
\newcommand{\Zset}{\mathbb{Z}}
\newcommand{\Qset}{\mathbb{Q}}
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Rsetp}{\mathbb{R}_{>0}}
\newcommand{\Rsetpo}{\mathbb{R}_{\ge 0}}

\newcommand{\powerset}{\mathcal P}
\newcommand{\nxt}{\mathrm{next}}
\newcommand{\cannot}{\bullet}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\dist}{\mathcal{D}}
\newcommand{\measures}{\mathcal{D}}%{\mathcal{M}}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\de}[1]{\mathit{d#1}}  %
\newcommand{\borel}{\mathfrak{B}}
\newcommand{\productfield}{\otimes}
\newcommand{\fr}{\mathit{frac}}  %frac(x)

\newcommand{\ex}{\mathrm{Exp}}

%%%%%%%%%%%%%%%  algorithms

\newcommand{\B}{E}
\newcommand{\choices}{\mathcal W}
\newcommand{\stable}{\textbf{stable}}
\newcommand{\corners}{\mathcal E}
\usepackage[noend]{algorithm2e}


%%%%%%%%%%%%%%%  bisimulation

\newcommand{\bisim}{\sim}
\newcommand{\hennessy}{\mathit{Hen}}
\newcommand{\larsenskou}{\mathit{LS}}
\newcommand{\fengzhang}{\mathit{FZ}}

\newcommand{\sigmafield}{\Sigma}

\newcommand{\states}{\mathit{S}}
\newcommand{\sta}{s}
\newcommand{\Sta}{X}
\newcommand{\statesfield}{\sigmafield(\states)}

\newcommand{\labels}{\mathit{L}}
\newcommand{\lab}{a}
\newcommand{\Lab}{A}
\newcommand{\labelsfield}{\sigmafield(\labels)}

\newcommand{\resolver}{\rho}

\newcommand{\fail}{\square}

\newcommand{\dis}{\mu}
\newcommand{\distwo}{\nu}
\newcommand{\Dis}{M}

\newcommand{\mea}{\mu}
\newcommand{\meatwo}{\nu}
\newcommand{\Mea}{M}

\newcommand{\statemeasuresfield}{\sigmafield(\measures(\states))}

\newcommand{\enabled}{\states}
\newcommand{\zeromeasure}{\vec{0}}
\newcommand{\statebisim}{\sim_{state}}
\newcommand{\distbisim}{\sim_{dist}}

\newcommand{\lifting}{\mathcal{L}}

\newcommand{\functorfin}{\heartsuit}
\newcommand{\functorinf}{\spadesuit}


\DeclareMathOperator{\convex}{conv}

%%%%%%%%%%%%%%%  game and its semantics

\newcommand{\act}{L}%{\mathbb{A}\mathrm{ct}^\tau}
\newcommand{\actnotau}{\mathbb{A}\mathrm{ct}}
%\newcommand{\acte}{\mathbb{A}\mathrm{ct}\setminus\{\tau\}}
\newcommand{\acte}{\mathbb{A}\mathrm{ct'}}
\newcommand{\hidden}{\act_{hid}}
\newcommand{\sync}{\act_{sync}}
% \newcommand{\tran}[1]{{}\mathchoice%
%     {\stackrel{#1}{\rightarrow}}
%     % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
%     {\mathop {\smash\rightarrow}\limits^{\vrule width 0pt height 0pt depth 1pt\smash{#1}}}
%     {\stackrel{#1}{\rightarrow}}
%     {\stackrel{#1}{\rightarrow}}
% {}}
% \renewcommand{\tran}[1]{\smash{\xrightarrow{#1}}}
\newcommand{\tran}[1]{{}\mathchoice%
    {\xrightarrow{#1}}
    % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
    {\smash{\xrightarrow{#1}}}
    {\xrightarrow{#1}}
    {\xrightarrow{#1}}
{}}
\newcommand{\itran}{\mathord{\hookrightarrow}}
\newcommand{\mtran}{\mathord{\rightsquigarrow}} %twoheadrightarrow

\newcommand{\acttran}[1]{{}\mathchoice%
    {\stackrel{#1}{\itran}}
% 
%     {\stackrel{#1}{\itran}}
    % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
     {\mathop {\smash\itran}\limits^{\vrule width 0pt height 0pt depth 4pt\smash{#1}}}
% 
    {\stackrel{#1}{\itran}}
    {\stackrel{#1}{\itran}}
{}}
\newcommand{\acttranlong}[1]{{}\mathchoice%
    {\stackrel{#1}{\itran}}
% 
%     {\stackrel{#1}{\itran}}
    % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
     {\mathop {\smash\itran}\limits^{\vrule width 0pt height 0pt depth 0pt\smash{#1}}}
% 
    {\stackrel{#1}{\itran}}
    {\stackrel{#1}{\itran}}
{}}
\newcommand{\probtran}[1]{{}\mathchoice%
    {\stackrel{#1}{\mtran}}
    % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
    {\mathop {\smash\mtran}\limits^{\vrule width 0pt height 0pt depth 4pt\smash{#1}}}
    {\stackrel{#1}{\mtran}}
    {\stackrel{#1}{\mtran}}
{}}
\newcommand{\probtranlong}[1]{{}\mathchoice%
    {\stackrel{#1}{\mtran}}
    % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
    {\mathop {\smash\mtran}\limits^{\vrule width 0pt height 0pt depth 0pt\smash{#1}}}
    {\stackrel{#1}{\mtran}}
    {\stackrel{#1}{\mtran}}
{}}
\newcommand{\Rightarrowtran}[1]{{}\mathchoice%
    {\stackrel{#1}{\Rightarrow}}
    % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
    {\mathop {\smash\Rightarrow}\limits^{\vrule width 0pt height 0pt depth 4pt\smash{#1}}}
    {\stackrel{#1}{\Rightarrow}}
    {\stackrel{#1}{\Rightarrow}}
{}}

\newcommand{\arrowsub}[1]{\hspace{-2pt}_{#1}}


\newcommand{\suc}{\mathrm{succ}}
\newcommand{\ext}{e}
\newcommand{\Mar}{M}
\newcommand{\suco}{{\suc_{\ext}}}
\newcommand{\sucm}{\suc_{\Mar}}
\newcommand{\suct}{\suc_{\tau}}
\newcommand{\rate}{\lambda}
\newcommand{\rates}{\mathrm{R}}
\newcommand{\prob}{\mathbf{P}}

\newcommand{\setofruns}{\mathbb{R}\mathrm{uns}}
\newcommand{\probm}{\mathcal{P}}
\newcommand{\expected}{\mathbb{E}}
\newcommand{\scheduler}{\mathfrak{S}}
\newcommand{\histories}{\mathbb{H}\mathrm{istories}} %in CE games
%\newcommand{\histories}{\mathbb{P}\mathrm{aths}} %in CE games
\newcommand{\history}{\mathfrak{h}} %in CE games
\newcommand{\dhistory}{[\mathfrak{h}]} %induced history in the discrete game
\newcommand{\paths}{\mathbb{P}\mathrm{aths}} %in IMC
\newcommand{\mypath}{\mathfrak{p}} %in IMC

\newcommand{\comp}[1]{\parallel_{#1}}
\newcommand{\hide}[1]{\diagdown{#1}}
\newcommand{\actt}{\act_\tau}

%%%%%%%%%%%%%%%%%%%%%% others

\newcommand{\eps}{{\varepsilon}}

\newcommand{\exponential}{\mathrm{Exp}}

\newcommand{\kernel}{\tau}
\newcommand{\kernelsp}{\kernel^{\sigma,\pi}_{\history_0}}

\newcommand{\trule}[3]{{\displaystyle{\frac{#1}{#2}}{\quad#3}}}

%%%%%%%%%%%%%%%%%% Probabilistic automata

\newcommand{\PA}{D}
\newcommand{\patrans}{\longrightarrow}

\newcommand{\patransa}[1]{{}\mathchoice%
    {\stackrel{#1}{\longrightarrow}}
    % vyskove uspornejsi varianta pro \textstyle, aby se nerozbijel radkovy rejstrik
    {\mathop {\smash\longrightarrow}\limits^{\vrule width 0pt height 0pt depth 4pt\smash{#1}}}
    {\stackrel{#1}{\longrightarrow}}
    {\stackrel{#1}{\longrightarrow}}
{}}

\newcommand{\pts}{\mathbf{P}}

%%%%%%%%%%%%%%%%%% Stochastic automata

\newcommand{\SA}{\mathcal{S}}
\newcommand{\locations}{\mathcal{Q}}
\newcommand{\clocks}{\mathcal{C}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\edges}{\rightarrow}
\newcommand{\clocksetting}{\kappa}
\newcommand{\clockdist}{F}

\newcommand{\loc}{q}
\newcommand{\clo}{c}
\newcommand{\Clo}{X}
\newcommand{\val}{\xi}

\newcommand{\loctop}{q}
\newcommand{\locleft}{u}
\newcommand{\locright}{v}
\newcommand{\locbottom}{r}

\newcommand{\reachablemeasures}{\mathcal{R_M}}

\newcommand{\chain}{\bar{\PA}}
\newcommand{\chainstates}{\bar{S}}
\newcommand{\SAstates}{S}

\newcommand{\abssemantics}{\hat{\pts}}
\newcommand{\absstates}{\hat{\states}}

\newcommand{\SSC}{\theta}
\newcommand{\sequences}{W}
\newcommand{\seq}{w}
\newcommand{\zone}{z}
\newcommand{\zones}{Z}
\newcommand{\domain}{D}
\newcommand{\dimensions}{X}

\newcommand{\refappendix}{Appendix}%{\cite{techrep}}

\setlength{\marginparwidth}{4.3cm}
\setlength{\marginparsep}{0.1cm}
\newcommand{\todo}[1]{\todoc{#1}{red}}
\newcommand{\todoc}[2]{%
  % Add to todo list
  %
  \begin{tikzpicture}[remember picture]%
      \node [coordinate] (inText) {};%
  \end{tikzpicture}%
  %
  % Make the margin par
  \marginpar{%
      \begin{tikzpicture}[remember picture]%
   %
          \draw node[draw=#2, color=#2, text width = 4.2cm, inner sep=2pt] (inNote)%
                   {{\footnotesize #1}};%
      \end{tikzpicture}%
  }%
  %
  \begin{tikzpicture}[remember picture, overlay]%
      \draw[draw = #2, thick]%
          ([yshift=-0.1cm] inText)%
              -| ([xshift=-0.1cm] inNote.west)%
              -| (inNote.west);%
  \end{tikzpicture}%
  %
}%
\renewcommand{\todoc}[2]{}
%
\newcommand{\holger}[1]{\todoc{Holger: #1}{WildStrawberry}}
\newcommand{\jena}[1]{\todoc{Jeňa: #1}{OliveGreen}}
\newcommand{\honza}[1]{\todoc{Honza: #1}{blue}}


\newcommand{\out}[1]{} %{#1}
\newcommand{\red}[1]{{\color{red} #1}}

\newcommand{\tableau}[1]{\textbf{#1}}

%%%%%%%%%%%%%%%%%% reftheorem


\newcounter{mycounter}
\newcommand{\theoremlike}[2]{\par\medskip\penalty-250\refstepcounter{theorem}{{\bfseries\noindent#2
\ref{#1}.}}}

\newcommand{\thmhelperpre}[2]{\theoremlike{#1}{#2}}
\newcommand{\thmhelperpost}{\par\medskip}

\newenvironment{reftheorem}[1]{\thmhelperpre{#1}{Theorem}}{\thmhelperpost}
\newenvironment{reflemma}[1]{\thmhelperpre{#1}{Lemma}}{\thmhelperpost}
\newenvironment{refobservation}[1]{\thmhelperpre{#1}{Observation}}{
\thmhelperpost}
\newenvironment{refcorollary}[1]{\thmhelperpre{#1}{Corollary}}{\thmhelperpost}
\newenvironment{refproposition}[1]{\thmhelperpre{#1}{Proposition}}{
\thmhelperpost }

%\newtheorem{claim}[theorem]{Claim}
%\theoremstyle{plain}
%\newtheorem{proposition}[theorem]{Proposition}




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \newcommand{\myspace}{\vspace*{-1em}}

==> odpad.tex <==


\section{Proofs from Section~\ref{sec:bisim}}

Recall $\functorfin(f)(n)(a)=(id\times\powerset(f))(n(a))$.

\begin{reflemma}{lem:fin-coin}
 The union of $\functorfin$-bisimulations %from Definition~\ref{def:finite-functor} 
and %the relational bisimulation 
$\bisim$ %s by Definition~\ref{def:finite-bisim} 
coincide.
\end{reflemma}
\begin{proof}
First, we prove that whenever there is $\functorfin$-bisimulation $(R,\overline\nxt)$ with $(\dis,\distwo)\in R$ then $\dis\bisim\distwo$ by proving that $R\cup R^{-1}$ is a bisimulation relation. Let $a\in\act$ and $\dis R \distwo$ or $\distwo R \dis$, wlog the former (the latter follows symmetrically).
\begin{enumerate}
 \item The first condition of the relational bisimulation follows by
\begin{align*}
\dis(S_a)&=\pi_1(\nxt(\dis)(a))\\
&=\pi_1(\nxt\circ\pi_1\langle\dis,\distwo\rangle(a))\\
&=\pi_1(\functorfin\pi_1\circ\overline\nxt\langle\dis,\distwo\rangle(a))\\ &=\pi_1((id\times\powerset\pi_1)(\overline\nxt\langle\dis,\distwo\rangle(a)))\\
&=id(\pi_1(\overline\nxt\langle\dis,\distwo\rangle(a)))\\
&=\pi_1((id\times\powerset\pi_2)(\overline\nxt\langle\dis,\distwo\rangle(a)))\\
&=\pi_1(\functorfin\pi_2\circ\overline\nxt\langle\dis,\distwo\rangle(a))\\
&=\pi_1(\nxt\circ\pi_2\langle\dis,\distwo\rangle(a))\\
&=\pi_1(\nxt(\distwo)(a))\\
&=\distwo(S_a)
\end{align*}
 \item For the second condition of the relational bisimulation, let $\dis\tran{a}\dis'$. Since
\begin{align*}
\dis'&\in\pi_2(\nxt(\dis))(a)\\
&=\pi_2(\nxt\circ\pi_1\langle\dis,\distwo\rangle(a))\\
&=\pi_2(\functorfin\pi_1\circ\overline\nxt\langle\dis,\distwo\rangle(a))\\
&=\pi_2((id\times\powerset\pi_1)\Big(\overline\nxt\langle\dis,\distwo\rangle(a)\Big))\\
&=\powerset\pi_1(\pi_2\Big(\overline\nxt(\langle\dis,\distwo\rangle)(a)\Big))
\end{align*}
there is $\distwo'$ with
$$\langle\dis',\distwo'\rangle\in \pi_2\Big(\overline\nxt(\langle\dis,\distwo\rangle)(a)\Big)$$
% We show that $\dis' R\distwo'$ since
% \begin{align*}
% \distwo'&\in\powerset\pi_2(\pi_2\Big(\overline\nxt(\langle\dis,\distwo\rangle)(a)\Big))\\
% &=\pi_2(id\times\powerset\pi_2\Big(\overline\nxt(\langle\dis,\distwo\rangle)(a)\Big))\\
% &=\pi_2(\functorfin\pi_2\Big(\overline\nxt(\langle\dis,\distwo\rangle)(a)\Big))\\
% &=\pi_2(\nxt(\pi_2(\langle\dis,\distwo\rangle))(a))\\
% &=\pi_2(\nxt(\distwo))(a)
% \end{align*}
Since $R$ is a coalgebra, we have $\langle\dis',\distwo'\rangle\in R$, i.e.\ $\dis'R\distwo'$.
\end{enumerate}

\medskip

Second, given $R=\mathord{\bisim}$, we define $\overline\nxt$ making it into a coalgebra such that the bisimulation diagram commutes. Let $\suc_a(\dis)=\{\dis'\mid\dis\tran{a}\dis'\}$ denote the set of all $a$-successors of $\dis$. For $\dis R\distwo$, we set
$$\overline\nxt(\langle\dis,\distwo\rangle)(a)=(\dis(S_a),\{\langle\dis',\distwo'\rangle\in R\cap \suc_a(\dis)\times\suc_a(\distwo)\})$$
Since we imposed $\langle\dis',\distwo'\rangle\in R$, $(R,\overline\nxt)$ is a $\functorfin$-coalgebra. Further, we prove the bisimulation diagram commutes. Firstly, 
\begin{align*}
\nxt\circ\pi_1\langle\dis,\distwo\rangle&=(\dis(S_a),\suc_a(\dis))\\ 
\nxt\circ\pi_2\langle\dis,\distwo\rangle&=(\distwo(S_a),\suc_a(\distwo))
\end{align*}
Therefore,
$$\pi_1(\nxt\circ\pi_1\langle\dis,\distwo\rangle)= \dis(S_a)=\pi_1(\functorfin\pi_1(\overline\nxt\langle\dis,\distwo\rangle)(a))$$
and
$$\pi_1(\nxt\circ\pi_2\langle\dis,\distwo\rangle)=\distwo(S_a)=\dis(S_a)= \pi_1(\functorfin\pi_2(\overline\nxt\langle\dis,\distwo\rangle)(a))$$
since $\dis(S_a)=\distwo(S_a)$ due to $\dis\bisim\distwo$ and the first relational bisimulation condition. Secondly,
\begin{align*}
\pi_2(\nxt\circ\pi_1\langle\dis,\distwo\rangle(a))&= \suc_a(\dis)\stackrel{(1)}=\pi_2(\functorfin\pi_1(\overline\nxt\langle\dis,\distwo\rangle)(a))\\
\pi_2(\nxt\circ\pi_2\langle\dis,\distwo\rangle(a))&=\suc_a(\distwo) \stackrel{(2)}=\pi_2(\functorfin\pi_2(\overline\nxt\langle\dis,\distwo\rangle)(a)) 
\end{align*}
After we show $(1)$ and $(2)$, we know both components of  $\functorfin\pi_1(\overline\nxt\langle\dis,\distwo\rangle)(a)$ are the same as of $\nxt(\pi_1\langle\dis,\distwo\rangle)(a)$, and similarly for $\functorfin\pi_2$, hence the commuting. As to $(1)$, $\supseteq$ follows directly by $\overline\nxt$ defined above. For $\subseteq$, for every $\dis'\in\suc_a(\dis)$ there is $\distwo'\in\suc_a(\distwo)$ with $\dis'R\distwo'$ due to the second realtional bisimulation condition. Thus also $\langle\dis',\distwo'\rangle\in \functorfin\pi_1 (\overline\nxt\langle\dis,\distwo\rangle)(a)$. $(2)$ follows from symmetric argument and $R$ being symmetric.
\end{proof}


\begin{reflemma}{lem:inf-coin}
The %greatest 
union of $\functorinf$-bisimulations and $\bisim$ coincide.
% The coalgebraic bisimulations from Definition~\ref{def:infinite-functor} and the relational bisimulations by Definition~\ref{def:infinite-bisim} coincide.
\end{reflemma}
\begin{proof}
The proof is similar, with applications to $a\in\act$ replaced by applications to $A\subseteq\act$.
\end{proof}


% \begin{refproposition}{prop:coin-on-pa}
% The bisimulations of Definition~\ref{def:finite-bisim} and Definition~\ref{def:infinite-bisim} coincide on PA.
% \end{refproposition}
% \begin{proof}
% Each bisimulation $R$ of Definition~\ref{def:infinite-bisim} is a bisimulation of Definition~\ref{def:finite-bisim}. Indeed, the conditions for $a$ follow by taking $A=\{a\}$. Further, each bisimulation $R$ of Definition~\ref{def:finite-bisim} is a bisimulation of Definition~\ref{def:infinite-bisim}. No, it is not. Indeed, consider $\dis(S_A)\leq\sum_{a\in A}\dis(S_a)$.
% \end{proof}





\section{Relational bisimulation}

An equivalence relation $\bisim \subseteq \states \times \states$ over states can be lifted to a relation $\lifting(\bisim) \subseteq \dist(\states) \times \dist(\states)$ over measure by letting $\mea \,\lifting(\bisim)\, \mea'$ if for each set of equivalence classes $\Sta \subseteq \states / \bisim$ such that $\bigcup \Sta$ is measurable we have $\mea(\bigcup \Sta) = \mea'(\bigcup \Sta)$.

\begin{definition}[Larsen\&Skou state-based bisimulation]
 We say that an equivalence $\bisim  \subseteq \states \times \states$ is a (strong) \emph{bisimulation} if for each $\sta \, \bisim \, \sta'$ and each
 $a \in \labels$ we have 
 \begin{enumerate}
  \item either $\kernel_a(\sta) = \zeromeasure = \kernel_a(\sta')$
  \item or $\kernel_a(\sta)  \, \lifting(R)\, \kernel_a(\sta')$.
 \end{enumerate}
\end{definition}

The largest state bisimulation is denoted by $\statebisim$.

\begin{definition}[Distribution strong bisimulation]
 We say that an equivalence $\bisim \subseteq \dist(\states) \times \dist(\states)$ is a \emph{distribution (strong) bisimulation} if for each $\mea \,\bisim\, \mea$ and each measurable $X \subseteq \labels$,
 \begin{enumerate}
  \item $\mea(\enabled_X) = \mea'(\enabled_X)$, and
  \item for each measurable $\rho : \enabled_X \to X$ there is a measurable $\rho': \enabled_X \to X$ such that 
%   
 $\mea_\rho \, \bisim \, \mea'_{\rho'}$ where 
  $$ \mea_\rho(A) := \mea(A \setminus X) + \int_X \kernel_{\rho(x)}(A) \cdot \mea(dx) \quad \forall A\in\statesfield. $$
 \end{enumerate}
\end{definition}

The largest distribution bisimulation is denoted by $\distbisim$.

% [asi potrebuju singletony meritelny]

\section{Co-algebraic bisimulation}

category $Mes$
\begin{itemize}
 \item objects: measurable spaces; for object $X$, let $\Sigma(X)$ denote its $\sigma$-algebra and we use $X$ also as the carrier set
 \item morphisms: measurable maps
\end{itemize}

functor $\Pi$
\begin{itemize}
 \item on objects: $\Pi(X)=\{\mu:\Sigma(X)\to[0,1]\mid \mu \text{ is a probability measure on } X\}$
 \item on morphisms: $\Pi(f)=\lambda \nu.\nu\circ f^{-1}$
\end{itemize}

% $\Pi(f)=\int f\de-$, \\i.e. $\Pi(f)=\lambda\nu.\int_{x\in X} f(x)\nu(\de x)$

category $\Pi(Mes)$ is the image of the endofunctor $\Pi$ on $Mes$

Let $A$ be fixed and $\mathcal P(A)$ denote the set of \emph{measurable} subsets of $A$

functor $F$
\begin{itemize}
 \item on objects: $F(X)=\big([0,1]\times X\big)^{\mathcal P(A)}$
 \item on morphisms: $F(f)=\big(id\times f\big)^{\mathcal P(A)}$
\end{itemize}

Let $S=(S,f_S)$ and $T=(T,f_T)$ be $F$-coalgebras in category $\Pi(Mes)$. A bisimulation of $S$ and $T$ is an object $R$ of $\Pi(Mes)$ \footnote{we may require the structure of a relation: $R\subseteq X\times Y$, or we can take categorical product in order to obtain the relation} that is an $F$-coalgebra equipped with $F$-coalgebra homomorphisms to $S$ and to $T$.

For $f:X\to F(X)$m and $B\in\mathcal P(A)$, let $\langle f^m_B,f^s_B\rangle:X\to [0,1]\times X$ denote the function equal to $f(-)(B)$, i.e. components of $f$.

Then the coalgebraci bisimulation definition requires:
\begin{itemize}
 \item $f^m_B(r)=f^m_B(\pi_1(r))$ and $f^m_B(r)=f^m_B(\pi_2(r))$, hence $f^m_B$ must be the same on both components of the bisimulation (if we consider the product, then for $sRt$ we have $f^m_B(s)=f^m_B(t)$)
 \item $f^s_B(r)=f^s_B(\pi_1(r))$ and $f^s_B(r)=f^s_B(\pi_2(r))$ and of course $f^s_B(r)\in R$, hence all these conditions must again hold for the element of bisimulation that contains the successors (if we consider the product, then for $sRt$ we have $f^s_B(s)\ R\ f^s_B(t)$)
\end{itemize}

Lemma: equivalent to relational


\section{Categorical bisimulation}

span of zig-zags because we have pullbacks (?)

\section{Algorithms}

computing gfp on distributions: if discretized what sort of error occurs? any $\varepsilon$-bisimulation studied in past?

computing gfp on states: HH used lifting to distributions, lift to measures for given time distributions ($\{Exp(r)\mid r\in\Rset\}\cup\cdots$)




\section{Bisimulation in compositional modelling}
\label{app:compositional}

[zatim bordel bez ladu a skladu]

For this subsection we fix a set of labels $\labels$.
% 
% We lift the bisimulation relation to probabilistic automata by endowing each PA $\PA$ with an initial distribution $\alpha$ and setting $\PA_1 \bisim \PA_2$ if $\alpha_1 \bisim \alpha_2$ in the disjoint union of the automata.

The key operation for compositional modelling is the \emph{parallel composition} operator. For $\PA_1 = (\states_1, \labels, \patrans_1)$, $\PA_2 = (\states_2, \labels, \patrans_2)$, and a subset of their labels $A \subseteq \labels$, let $\PA_1 \parallel_A \PA_2$ denote their (CSP style) parallel composition $(\states_1 \times \states_2, \labels, \patrans)$ where $(\sta_1,\sta_2) \patransa{\lab} \dis$ if $\dis = \dis_1 \times \dis_2$ (The product distribution $\dis_1 \times \dis_2$ assigns $\dis_1(\sta_1') \cdot \dis_2(\sta_2')$ to all $(\sta_1',\sta_2')$.) and 
\begin{itemize}
 \item $\lab\in A$, $\sta_1 \patransa{\lab}\arrowsub{1} \, \dis_1$, and $\sta_2 \patransa{\lab}\arrowsub{2} \, \dis_2$; or \hfill {\footnotesize (synchronous move)}
%  such that $\dis = \dis_1 \times \dis_2$, i.e. $\dis((\sta_1',\sta_2')) = \dis_1(\sta_1') \cdot \dis_2(\sta_2')$ for all $\sta_1',\sta_2'$; or
\item $\lab\not\in A$, $\sta_1 \patransa{\lab}\arrowsub{1} \, \dis_1$ and $\dis_2(\sta_2) = 1$, or $\sta_2 \patransa{\lab}\arrowsub{2} \, \dis_2$ and $\dis_1(\sta_1) = 1$.\hfill {\footnotesize (asynchronous move)}
% where $\delta_\sta$ assigns $1$ to $\sta$ and $0$ elsewhere.
% 
%  \item $\lab\not\in\labels$, $\sta_1 \patransa{\lab}\arrowsub{1} \, \dis_1$ and $\dis = \dis_1 \times \delta_{\sta_2}$, or $\sta_2 \patransa{\lab}\arrowsub{2} \, \dis_2$ and $\dis = \delta_{\sta_1} \times \dis_2$ where $\delta_\sta$ assigns $1$ to $\sta$ and $0$ elsewhere.
\end{itemize}
For distributions $\dis_1$, $\dis_2$ in probabilistic automata $\PA_1$, $\PA_2$, we denote by $\dis_1 \parallel_A \dis_2$ the distribution $\dis_1 \times \dis_2$ in $\PA_1 \parallel_A \PA_2$.

For bisimulation to be applicable in compositional modelling, it needs to be a congruence w.r.t. parallel composition. 

\begin{theorem}
Let $\dis_1,\dis_2$ be distributions in $\PA$ such that $\dis_1 \bisim \dis_2$.
We have $\dis_1 \parallel_A \dis \; \bisim \; \dis_2 \parallel_A \dis$ for any $\dis$ in $\PA'$ and $A\subseteq\labels$.
% Let $\dis_1$ and $\dis_2$ be distributions such that over states of a PA $\PA$ such that $\dis_1 \bisim \dis_2$. For any $\PA$ and we have $\PA_1 \parallel_A \PA \bisim \PA_2 \parallel_A \PA$.
%  Let $\PA_1$ and $\PA_2$ be automata such that $\PA_1 \bisim \PA_2$. For any $\PA$ and $A\subseteq\labels$ we have $\PA_1 \parallel_A \PA \bisim \PA_2 \parallel_A \PA$.
\end{theorem}

\section{Defs for expolynomials}


---

Let $\sequences$ be the set of all sequences (of length at most $k$) of the form $\seq = (a_1,c_1) \ldots (a_n,c_n)$ where each $a_i \in \actions$ and $c_i \in \clocks \cup \{\bot\}$ such that each clock appears at most one in the sequence, i.e. $c_i = c_j$ implies $i=j$ or $c_i = c_j = \bot$. 

From a state $s=(q,\SSC)$, each sequence encodes a possible execution to some state $(q',\SSC')$  -- a sequence of transitions with actions $a_i$ that may occur from $s$ before all the clocks active\jena{def} in $\SSC$ get below zero or get resampled. The elements 
$c_i$ encode which of the clocks active in $\SSC$ triggered the transition ($c_i$ is $\bot$ if the transition is triggered by a clock not active in $\SSC$ or a by a clock that is resampled earlier on the sequence). By a forward reachability. 

Traversing the sequence $\seq$ backwards from $q'$ in the qualitative TA model\jena{def} gives a \emph{zone} $\zone_{\seq,q}$, a symbolical representation of all clocks values in $q$ from that it is possible to perform this sequence. For each sequence $\seq$, we denote by $\zones_\seq$ the minimal set of zones
\begin{itemize}
\item that is a partition, i.e. for any $\zone_1,\zone_2 \in \zones_\seq$ we have $\zone_1 \cap \zone_2 = \emptyset$, and  
\item each zone $\zone_{\seq,q} \cap \domain(\SSC)$\jena{def domain} for $(q,\SSC)\in\states_\SA$ is a union of elements of $\zones_\seq$.\jena{def stavy grafu}
\end{itemize}
For each zone $z \in \zones_\seq$ and distribution $\SSC$ such that $\SSC(z) > 0$, we denote by $\SSC^z$ the conditioned distribution on $\domain(\SSC) \cap z$, i.e. for each measurable set $A$ in its support we have $\SSC^z(A) = \SSC(A)/\SSC(z)$.

For each sequence $\seq = (\act_1,\clo_1) \cdots (\act_n,\clo_n)$ and each action $\act$, let $\#_{\seq,\act} = \{i \mid \act = \act_i, \clo_i \neq \bot \}$ denote the number of times an active clock triggers the action $\act$ on the sequence $\seq$. The space of the sequence $X_\seq$ is $\prod_{\act\in\actions} (\Rsetpo)^{\#_{\seq,\act}}$ 
%
Finally, for each state distribution $\SSC^z$ over $z \subseteq (\Rsetpo)^\clocks$ we denote by $\SSC^z_\seq$ the distribution over $X_\seq$ obtained from $\SSC^z$ by projecting out all clocks not appearing in this sequence and mapping the dimension of each clock $\clo$ to the $i$-th dimension of $\act$ where $\clo$ appears in $\seq$ with the $i$-th occurrence of $\act$.

Let $\dimensions = \{(q,\SSC^z_\seq) \mid q\in\locations, (q,\SSC)\in\states_\SA, \seq \in\sequences, z \in \zones_\seq)\}$ be all different measures in the system induced by all sequences and zones of the sequences. To each state $(\loc,\SSC)$ we assign a discrete distribution $\dis_{(\loc,\SSC)}$ over $\dimensions$ that assigns to each $(\loc,\SSC^z_\seq)\in\dimensions$ probability $\SSC(z)/\SSC(\bigcup \zones_\loc)$ where $\zones_\loc = \bigcup_{\seq\in\sequences} \zones_{\seq,\loc}$.

